Xenos: Dataflow-Centric Optimization to Accelerate Model Inference on Edge Devices

Edge computing has been emerging as a popular scenario for model inference. However, the inference performance on edge devices (e.g., Multi-Core DSP, FGPA, etc.) suffers from inefficiency due to the lack of highly optimized inference frameworks. Previous model inference frameworks are mainly developed in an operator-centric way, which provides insufficient acceleration to edge-based inference. Besides, the operator-centric framework incurs significant costs for continuous development and maintenance. In this paper, we propose Xenos, which can automatically conduct dataflow-centric optimization of the computation graph and accelerate inference in two dimensions. Vertically, Xenos develops operator linking technique to improve data locality by restructuring the inter-operator dataflow. Horizontally, Xenos develops DSP-aware operator split technique to enable higher parallelism across multiple DSP units. Our evaluation proves the effectiveness of vertical and horizontal dataflow optimization, which reduce the inference time by 21.2\%--84.9\% and 17.9\%--96.2\% , respectively. Besides, Xenos also outperforms the widely-used TVM by 3.22$\times$--17.92$\times$. Moreover, we extend Xenos to a distributed solution, which we call d-Xenos. d-Xenos employs multiple edge devices to jointly conduct the inference task and achieves a speedup of 3.68x--3.78x compared with the single device.

==> algo/link.tex <==
\begin{algorithm}[!htbp]
\small
\makeatletter
\NewDocumentCommand{\LeftComment}{s m}{%
  \Statex \IfBooleanF{#1}{\hspace*{\ALG@thistlm}}\(\triangleright\) #2}
\makeatother

\algdef{SE}[EVENT]{Event}{EndEvent}[1]{\textbf{upon}\ \textsc{\small #1}\ \algorithmicdo}{\algorithmicend\ \textbf{event}}%
\algtext*{EndEvent}
\caption{Operator fusion and linking}
\label{algo:link}
\hspace*{\algorithmicindent} \textbf{Input}: 

\hspace*{\algorithmicindent}
\emph{\textbf{inGraph:}}{The input computation graph}

  \begin{algorithmic}[1]
      \For {Op $\in$ inGraph's operators}
        \If {Op.predecessors.size == 1}
            \State PrevOp = Op's predecessor
            \If {PrevOp and Op are fusable}
                \State Fuse PrevOp and Op in inGraph
            \EndIf
            \If {\Call {Linkable}{PrevOp, Op} }
                \State Link PrevOp and Op in inGraph
            \EndIf
        \EndIf
      \EndFor
    
    \Function {Linkable}{PrevOp, Op}
        \State ParamSize = PrevOp.parameters.size + Op.parameter.size
        \State \Return ParamSize $\leq$ $threshold$
    \EndFunction
  \end{algorithmic}
\end{algorithm}

==> algo/operator-partition.tex <==

\begin{algorithm}[!t]
\small
\makeatletter
\NewDocumentCommand{\LeftComment}{s m}{%
  \Statex \IfBooleanF{#1}{\hspace*{\ALG@thistlm}}\(\triangleright\) #2}
\makeatother

\algdef{SE}[EVENT]{Event}{EndEvent}[1]{\textbf{upon}\ \textsc{\small #1}\ \algorithmicdo}{\algorithmicend\ \textbf{event}}%
\algtext*{EndEvent}
\caption{DSP-aware Operator Partition (DOP)}
\label{algo-spe}
\hspace*{\algorithmicindent} \textbf{Input}: 

\hspace*{\algorithmicindent}
\emph{\textbf{inH: }}{The input height of the feature map.}

\hspace*{\algorithmicindent}
\emph{\textbf{inW: }}{The input width of the feature map.}

\hspace*{\algorithmicindent}
\emph{\textbf{outC: }}{The number of output channels (operator parameters)}

\hspace*{\algorithmicindent}
\emph{\textbf{K}}\textbf{[$1\dots outC$]:} {The list of kernels}

\hspace*{\algorithmicindent} 
\emph{\textbf{F}}\textbf{[$1\dots inH$] [$1\dots inW$] [$1\dots inC$]: }{The input feature map, \hspace*{\algorithmicindent} size of $inH\times inW\times inC$.}

\hspace*{\algorithmicindent} \emph{\textbf{P: }}{The expected parallelism degree, i.e. the number of DSP \hspace*{\algorithmicindent} units available on the edge device.}

  \begin{algorithmic}[1]
  \Event{\text{receiving} (\emph{K, F})}
      \hspace*{\algorithmicindent} \LeftComment{While receiving a feature map $F$ and the target operator (kernels) $K$, we output a partitioned $scheme$. We assume $P$ is global constant}
    \State $scheme=$ \textsc{fmp-algo}($K, F, P$)
    \State Forward $scheme$ to Inference Engine
  \EndEvent
  
 
     \Function{dop-algo}{$K, F, P$}
        \LeftComment{$scheme$ is encoded as a dictionary, with key as the } \LeftComment{core-id and value as the partitioned operators and} \LeftComment{feature map (fmp) assigned to this core }
        \For{$i$ $\gets$1 to $P$}
         \Comment{Initialization of $scheme$}
            \State $scheme$[$i$]=$\{op:\{\}, fmp:\{\}\}$
           
        \EndFor
        
        \LeftComment{Partition by output channel $outC$}
        \State $sliceByC=\lfloor outC/P \rfloor$
        \For{$i\gets$1 to $P$}
        \LeftComment{{\small $K$[$k_1:k_2$]  represents a slice in $K$, ranging from $k_1$ to $k_2$}}
            \State $k_1=\emph{sliceByC}\times(i-1)+1$
            \State $k_2=k_1+sliceByC$
            \State $scheme$[$i$][\emph{op}].append($K$[$k_1$:$k_2$])
            \State
            $scheme$[$i$][\emph{fmp}].append($F$)
        \EndFor
        
        \State $restC=sliceByC\times P+1$ 
        \LeftComment{Partition by input height $inH$}
        \State $K'=\emph{K}$[\emph{restC}:\emph{outC}]
        \State $sliceByH=\lfloor inH/Pn \rfloor$
        \For{$i\gets$1 to $P$}
            \State $h_1=\emph{sliceByH}\times(i-1)+1$
            \State $h_2=h_1+sliceByH$
            \State $scheme$[$i$][\emph{op}].append($K'$)
            \State
            $scheme$[$i$][\emph{fmp}].append($F$[$h_1$:$h_2$][:][:])
        \EndFor
        
        \State $\emph{restH}=\emph{sliceByH}\times P+1$ 
        \LeftComment{Partition by input width $inW$}

        \State $\emph{sliceByW}=\lfloor inW/P \rfloor$
        \State $F'=F[restH:outH][:][:]$
        \For{$i\gets$1 to $P$}
            \State $w_1=\emph{sliceByW}\times(i-1)+1$
            \State $w_2=w_1+\emph{sliceByW}$
            \State $scheme$[$i$][\emph{op}].append($K'$)
            \State
            $scheme$[$i$][\emph{fmp}].append($F'$[:][$w_1$:$w_2$][:])
        \EndFor
        
        
        \LeftComment{Randomly assign the remaining feature map}
        \State $\emph{restW}=\emph{sliceByW}\times P+1$
        \For{$i$ $\gets$ $restW$ to $inW$}
            
            \State $\emph{F''}=$$F$[:][$i$][:] \Comment{Pick the $i$th column of $F$}
            \State $r$=\textsc{rand}()$\%W$
            \Comment{Assign to a random DSP unit}
            \State $scheme$[$r$][\emph{op}].append($K'$)
            \State  $scheme$[$r$][\emph{fmp}].append($F''$) 
            
        \EndFor
    \State \Return $scheme$
     \EndFunction
  \end{algorithmic}
\end{algorithm}

==> coverletter.tex <==
\raggedend
{\section*{Cover Letter}}
\setcounter{section}{0}
Thanks for all the comments from the reviewers. Based on the revision suggestions and our internal discussion, we address the questions from the reviewers, with reference to the related part in our paper (\rv{The revised part in our paper is colored in red}).

\section{\text{Difference from TASO ( Reviewer 1, O1)}} 

TASO also supports typical split/combination of operators. However, \sysname supports more advanced fusion/split methods (PHF and HVF), incuding the fusion of Conv+BN+Relu, Conv+MaxPooling, and the inter-BN fusion. To the best of knowledge, such fusion has not been supported by TASO, although such fusion can be very effective in LNN acceleration.

More importantly, TASO's major contribution lies in the automatic optimization with computation graph, i.e. it automatically searches for equivalent sub-graphs to replace the original one, so that the ML training/inference can be accelerated. Just as we explained in \rv{\S\ref{black-vs-white} of the paper}, \textbf{such an optimization strategy is considered as a blackbox strategy, without considering hardware conditions.} Compared with \sysname's split/fusion, which is a whitebox strategy, TASO suffers from two major deficiencies. 

(1) TASO's fusion/split optimization is coarse-grained. For example, when it comes to memory optimization, it only targets at reducing the overall amount of memory consumption (it does not care about data locality as our IDR does). By contrast, \sysname's split/fusion is finer-grained and it optimizes memory for every layer with reference to the memory hierarchy. TASO, without awareness of such context information, will not do such finer-grained optimization. 

(2) TASO's optimization strategies can only work on a very small number of operators, and cannot scale. Since its search space can blow up very easily and its DFS algorithm will become unbearably slow. \sysname, however, eschews the blind enumeration and search because it knows hardware information and it uses the hardware information to help make partition decisions, therefore, it can scale to much larger computation graphs.


According to our discussion with the author of PET~\cite{osdi21_pet} (who also has great expertise in TASO), the scalability of the automatic optimization is always a headache issue for TASO and PET. The blackbox-like optimization is orthogonal to the whitebox-like optimization of \sysname. One is independent of external knowledge and conduct general (but inefficient) enumeration search whereas the other leverages the knowledge and conducts rule-guided search. \textbf{From this perspective, TASO and \sysname represent two completely different approaches, but they are complimentary.} In fact, the PET team is also considering integrating whitebox-like optimization to help improve the search efficiency. After all, with some hardware knowledge as guidelines, the search should be more efficient than blind enumeration.   


\section{External baseline on GPU machine (Reviewer 1, O2; Reviewer 2, O3)}

We have run the inference tasks and added the performance stats (refer to  \rv{\S\ref{gpu-stats}}). Just as mentioned  in the previous feedback, we do not expect \sysname to outperform the GPU-based solution. But it is worthwhile to understand the performance gap between \sysname-accelerated inference and the inference conducted in resource-abundant environment. 

Generally speaking, the inference of vanilla solution on ZCU is slower than the inference on GPU by an order of magnitude. But the inference time on ZCU becomes comparable to (and even slightly better than) that on GPU with \sysname acceleration. On the other hand, the inference on TMS is still slower than the inference on the GPU machine by one or two order of magnitude, even after \sysname acceleration (TMS is too resource-constrained!).


\section{APIs (Reviewer 1, O4)}
We have illustrated the APIs in the revised paper (refer to \rv{Table~\ref{xenos-op}}). \sysname has covered most operators in the mainstream ML systems. The current version of \sysname still requires some manual effort to adapt to the hardware, but we are working towards automatic deployment. We expect to support semi-automatic deployment after a few iterations in the near future and the final version \sysname should support automatic deployment. 

\section{Clarification of the Extensibility of \sysname (Reviewer 1, O5)}

We have implemented all the operators in C/C++, and most operators in assembly. The future iteration will continue to complement the operator library. 

Although nowadays there are hundreds of different operators, a large part of them can be reduced to several basic operators. For example, different convolution operators are actually encapsulated with the basic conv operator but with other different parameters. Besides, we also implement additional split/fuse operators in \sysname, which have not been supported by other ML systems. \textbf{and we only maintain one version of implementation and the vendor is expected to provide an adaption middleware (e.g HLS) to ease the deployment of Xenos.}

\section{Justification of Small LNN Partition (Reviewer 2, O1)}

\emph{small} or \emph{big} is pair of relative concepts. Though, compared with typical CNN models, LNN has pruned much and its parameters have been reduced. However, \textbf{the hardware resource can be more scarce. Compared with the resource amount, the model is still considered as too big, and the inference is still too slow without partition.} 

Following Reviewer 2's suggestion in the reply to our last feedback (``I suggest adding an experiment of running multiple inference tasks. One method is to parallelize tasks over multiple cores (without partition), and another method is to use all cores for each inference task (with partition). ''), we run 8 MobileNet inference tasks on the 8 cores of TMS320C6678, and each core undertakes one complete inference task. In this case, the AT reaches 213.3$\pm$0.001 seconds, which is much worse than the partitioned solution (As shown in Figure~\ref{6678AT}, even the vanilla partitioned solution can reach 833ms, which is faster than the unpartitioned solution by 2-3 orders of magnitude.). Such characteristics are different from the resource-abundant environment such as GPU cluster, where the batch processing can usually earn some performance benefit. On the DSP platforms, the L2 memory is very scarce, and cannot hold every layer of parameters (although the LNN is smaller than CNN, it is still too big for DSP platforms), so there will be frequent data migration from low-level storage to high-level storage, which costs significant overheads and slows down the inference. 

Besides, we choose to describe this micro-bench experiment in \rv{\S\ref{sec-model-partition-inefficiency}} instead of deferring it to the evaluation section, because the bad performance of unpartitioned model serves as the motivation of our HAP design. Therefore, it is more logical to mention it earlier in the paper.

\section{Clarification of IDR (Reviewer 2, O2)}

We have replaced the original illustrative figure with a simpler example (\rv{Figure~\ref{Restructure}}). We guess our previous example is still too complex and the description has some redundancy. In this revision, we explain the IDR with a fusion operator of conv1x1+max-pooling, which is probably the simplest fusion example in our library. The strategy is easy to explain: Previously, the inference is unaware of the data flow, so it blindly places the feature map in the memory, usually placing the matrix one by one. \textbf{This is inefficient, because the inference computation does not access the data matrix by matrix, instead, the conv1x1 computation accesses one element from each matix every time, and the max-pooling (stride of 2) computation scans 2x2 square every time.} Therefore, we have clearly drawn the magnified data access on the right hand of \rv{Figure~\ref{Restructure}}, the data flow goes through the four colored matrices (due to the conv computation), but if you look at the dataflow towards the face of one matrix (e.g. the red one), it follows the zigzag pattern (due to the max-pooling computation). \textbf{Our IDR leverages the knowledge of data access pattern by pre-encoding, so it restructures the dataflow for better locality.} Compared with the non-resturretured dataflow, the data can be fetched more efficiently.

Besides, \S\ref{sec-dataflow-inefficiency} is another example for IDR, which illustrates with only one conv1x1 kernel (without operator fusion). We think these two examples will help the readers to understand IDR.

\section{Clarification of HAP (Reviewer 3, O1 )}
We have updated our algorithm of HAP (refer to \rv{Algorithm~\ref{algo-spe}}). We redefine the variables, reorganize the workflow, and add more explanatory comments. We expect the revised algorithm should be more concise. 

The main idea of the algorithm is the triple partition, first by output channel, then by input height, and finally by input width. The $outC$-based partition is actually the partition of operator kernels. It is very similar to the data parallelism in typical machine learning.
The $inH$- and $inW$-based partition is actually the partition of the feature map. It is very similar to the model parallelism in typical machine learning. The partition is rule-based and the ``rule'' here is the hardware constraints (mainly the computation units). With this in mind, we think it will be much easier to understand HAP in \sysname.


\section{\sysname's generalization to other models (Reviewer 3, O2)}

Following Reviewer 3's suggestion, we add the extensive experiments (refer to \rv{\S\ref{xenos-general}}) on two other models, which are popular in objection detection scenarios, i.e. CenterNet and LSTM. Our evaluation on TMS platform further demonstrates \sysname can  also effectively accelerate the inference task based on these models.


\section{Conclusion}
We are really grateful to the shepherding discussion from all reviewers. Reviewer 2 and Reviewer 3's suggestions help us to improve the algorithm and make the experiments more persuasive. We are especially thankful to Reviewer 1 for his/her inspiring reminder on TASO-related comparison, which leads us to discuss it with the TASO expert/PET author. The discussion leads us to view \sysname's differentiation from TASO/PET in a much higher level (Even ourselves have not thought of \sysname in such a high level before). The combination of blackbox-like and whiltebox-like optimization probably will become a future trend in typical ML systems. After all, blackbox-like optimization has come to the bottleneck due to its search inefficiency and TASO/PET have to resort to external knowledge for whitebox-like optimizations. We feel excited that \sysname is moving a step in this promising direction, and we also believe more influential work will come out following this direction.   






==> d-xenos-3.tex <==
\section{Distributed Inference} 
\label{sec-distributed-inference}

\input{algo/dist-enumerate}
As the model size grows increasingly large, we envision that the inference workload can soon go beyond the capacity of single edge devices. Recent models, such as ResNet-101 (60.2M)~\cite{cvpr16-resnet}, Bert (340M$\sim$481000M)~\cite{devlin2018bert} and GPT-3\cite{radford2018improving}(175000M), can hardly be used for single-device inference, making distributed inference become a necessity.
Driven by these current and future scenarios, we extend \sysname to leverage multiple devices for joint inference computation, and we call the distributed version of \sysname as \dsysname. 

The key idea of \dsysname is to incorporate both model-parallel computation and  parameter synchronization among multiple devices, to cut down the overall inference time. 
However, we note that, compared with \sysname, \dsysname may not achieve optimal inference time if it still follows the priorities of OP (\S\ref{sec-ha-strategy}) to partition the feature map. 
Taking convolution operator as an example, recall that convolution's OP priorities \emph{outC}-based partition over \emph{inH}-/\emph{inW}-based partition. 
The reason is \emph{outC}-based partition can fully leverage the shared memory across different DSP units and avoid padding overheads due to  \emph{inH}-/\emph{inW}-based partition. 
However, when it comes to \dsysname, different edge devices do not shared memory, and it can hardly tell whether or not \emph{outC}-based partition can outperform \emph{inH}-/\emph{inW}-based partition.
Therefore, \dsysname needs to balance two types of overheads, i.e., the communication overheads due to parameter synchronization and the computation overheads due to imbalanced partition \hw{I do not see how we balance these two types of overheads. To my understanding, we only try to partition the operator as balance as possible, without considering the communication overhead.}. 
To address this problem, \dsysname uses a tree based traversal algorithm to determine the partition strategies.

The general enumeration algorithm is described in Algorithm~\ref{algo:enumerate}. \dsysname enumerates every possible combination of  partition schemes \hw{We do not define ``partition schemes'' before. I was trying to add it in \Cref{algo:enumerate} but failed.} towards dimensions appeared in feature maps or operator parameters involved in the inference, which can reach $d!$ different combinations at most if there are totally $d$ dimensions.
For example, there are three dimensions in matrix multiplication ($m$, $n$, and $k$, where $k$ is shared by both feature map and parameter) and seven dimensions in convolution ($batch$, $inC$, $inH$, $inW$, $outC$, $r$ and $s$, where $inC$ is shared by both feature map and parameter). \hw{I am not sure if we should give such a detailed definition of ``dimension''. Actually, this is also not a very formal definition.}
However, as we discussed in \S\ref{sec-ha-strategy} that \sysname only partitions along certain dimensions, \dsysname also chooses these dimensions to partition \cred{because we empirically notice that the other dimension-based partition (e.g. $inC$-based partition for convolution operator) cannot achieve better performance in the distributed setting either.} 
Therefore, \dsysname still focuses on the partition schemes along \emph{inH}, \emph{inW} and \emph{outC} when partitioning a convolution, as shown in Figure~\ref{fig-branch-partition}.
Then \dsysname chooses the best partition strategy among them according to the profiling result of their execution time.
Due to such search process is one-off for each model when deploying on a specific platform, the search cost is acceptable.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{fig/branch-partition.pdf}
    \caption{Enumerating partition schemes in \dsysname}
    \label{fig-branch-partition}
    \vspace{-0.2cm}
\end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{fig/partition-tree.pdf}
%     \caption{Partition tree in \dsysname 
%     \hw{I think we may use a algorithm instead of a figure to illustrate how we perform the tree-based traversal partition search? Then we can also keep \Cref{fig-branch-partition} as an example}}
%     \label{fig-partition-tree}
%     \vspace{-0.5cm}
% \end{figure}

==> design-bk.tex <==
\section{Design of Xenos}
\label{sec-design}

\subsection{Architecture and Workflow}

\Cref{arch} illustrates the architecture of \sysname. \sysname consists of two modules, a {\it hardware-adaptive model optimizer} and an {\it inference engine}. Given an NN model to be optimized, the model optimizer will first conduct an offline optimization with reference to the edge hardware constraints, and then output an optimized model, which is equivalent to the original model. The inference engine is fed with the input data and the optimized model, then it employs multiple DSP units to execute the inference task. The inference engine outputs the inference result to the applications, as well as a profiling report for engineers to conduct further performance analysis and optimization. 

As the key module in \sysname, the model optimizer includes four main components, namely, Efficient Memory Pool Group (EMPG), Operator Elastic Combiner (OEC), Feature Map Partitioner (FMP), and Inter-operator Dataflow Restructurer (IDR). 
% \hw{I changed it to IDR as we discussed. Check other place.} 
% \cb{The optimizer mainly optimize the data organization of the model, thus improve the performance.}
% \hw{I am thinking if \sysname{}'s main contribution is to optimize the \*dataflow\* of the inference model. OEC, FMP and IDR optimize the dataflow of parameters and feature maps, but actually also change the computation graph, e.g., operator split and operator fusion.}
The optimizer optimizes the data organization in two aspects. 
OEC and FMP reorganize the parameters and feature maps based on {\it hardware adaptive partition} (HAP) to fit into the memory hierarchy organized by EMPG, and IDR restructures the dataflow to achieve better data locality, thus the parameters and feature maps can be efficiently accessed by the inference engine.
% It relies on OEC to optimize the parameters (e.g. the weight tensors of the operators), and relies on FMP and IDR to optimize the feature maps. 
% After the optimization, the parameters and feature maps can be well fit into the memory hierarchy organized by EMPG: 
% Parameters are well cached by each DSP core's L2 cache, and feature maps are partitioned and stored in shared memory, thus they can be efficiently accessed by the inference engine.
% with good data locality. 
% We explain the four components in more detail.


\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{fig/xenos_arch.pdf}
	\caption{The architecture of \sysname}
	\label{arch}
	\vspace{-0.5cm}
\end{figure}

% ToDO: remove Image parititoner and Parameter Partitoner. SPE is reposible for feature map partition, OEC is responsible for parameter partition. 

% \textbf{EMPG and Coordinator logic.} 
% EMPG serves as the main storage in \sysname, and it organizes multiple types of storage media in a hierarchical way. EMPG has been integrated with an elaborate mechanism to reasonably allocate and reuse memory for different types of data. Both the input image data and the loaded model parameters are stored in EMPG. The Coordinator serves as the main bridge to communicate EMPG with other modules. It is responsible for distributing the divided data of IP and PP to the DSP units for inference computation. Meanwhile, it is also responsible for coordinating and storing temporary data generated during the inference process. Besides, for the sake of efficiency, Coordinator carefully manages the data cache and overlaps the data communication and inference computation in the workflow.

%\hwsay{Reconstruct this subsection.}

\para{EMPG} is the main storage for \sysname, which organizes L2 memory and SRAM-based shared memory in a hierarchical way. 
Since the under-optimized model may generate too large parameters and feature maps to well fit in the memory hierarchy, \sysname relies on the other three components (OEC, FMP and IDR) to optimize the data storage and dataflow to achieve memory efficiency.

\para{OEC} reorganizes the parameter storage by performing operator linking and operator split, as well as operator fusion.
Operator linking further reduces the redundant memory access by considering the complex dataflow which cannot be optimized by operator fusion.
Operator split uses HAP to split the parameters to fit them into the private L2 memory for each DSP unit (detailed in \S\ref{sec-op-reshape}).

% \cred{\para{OEC} can fuse/split the parameters in the model. In the under-optimized model, some operators involve redundant computation, whereas the others may have too large-sized parameters to fit into L2 cache. OEC conducts elastic fusion/split for these operators to accelerate the computation and improve memory efficiency (detailed in \S\ref{sec-op-reshape}). }
% \hw{to be removed}

% \para{OEC} \hw{\textit{logically} fuses and splits the operators improve the memory efficiency.
% Different with typical fusion and split optimizations, \sysname{} does not generate the fused or splitted operators due to the limitation of operator library for edge devices.
% Instead, \sysname{} achieves similar optimization by reorganizing the model parameters, which will be illustrated in \S\ref{sec-op-reshape}.
% }

\para{FMP} uses HAP to generate the partition scheme of the feature maps according to the DSP units. The scheme enables each DSP unit to be assigned with a partitioned feature map in load balance, and these DSP units can execute in high parallelism with the partitioned feature maps (detailed in \S\ref{sec-ha-strategy}). 

\para{IDR} defines the data layout of the feature maps when they are output to the shared memory. As mentioned in \S\ref{sec-dataflow-inefficiency}, the inference engine can suffer from lots of compulsory cache misses without considering the data layout of the feature maps. Targeting at this, IDR restructures the dataflow between adjacent operators linked by OEC, so that the feature maps output from the previous operator can be accessed by the subsequent operator in good locality
(detailed in \S\ref{sec-dr-strategy}).
% \hw{According to our new story, IDR should also consider the logical transformation result of OEC (which we actually do). fig 3 should also be revised.}

The following subsections give the design detail of each component in \sysname{}.

% \textbf{IE} executes the inference computation with the optimized operators (by OEC) and the partitioned feature maps (by FMP). More specifically, multiple DSP cores jointly execute the inference task. Each DSP core reads the assigned feature map from the shared memory and reads the related operator parameters from its L2 cache. The feature maps, whose layout has been restructured by DR, can be sequentially accessed with good spatial locality. The operator parameters, which have been optimized by OEC and well fit into the L2 cache, can be accessed even faster than the feature maps.   


% \textbf{RD} serves as an extension module for \sysname. It captures the profiling metrics during the inference and generates reports. The profiled metrics include memory cost, computing resource cost, and the time cost (such as the total time cost and the individual time cost of each module). Engineers refer to the profiling reports to identify the bottleneck and conduct deeper optimization.


% \para{Coordinator} 
% serves as the main bridge to communicate EMPG with other modules. 
% It is responsible for distributing the divided data of IP and PP to the DSP units for inference computation. 
% Meanwhile, it is also responsible for coordinating and storing temporary data generated during the inference process. 
% Besides,
% % for the sake of efficiency,
% Coordinator carefully manages the data cache and overlaps the data communication and inference computation in the workflow \hw{to achieve better performance}.
% \hwsay{Not sure if `for the sake of' is proper in written English.}

%DR is mainly responsible for the Inter-layer Aware Dataflow Scheduling. According to the calculation type of the inter-layer operator, this module can realize the fine-grained data arrangement, which allows part of edge hardwares to improve the inference performance through more efficient data reading operations. In MP, the Operator Elastic  Combination( OEC) module can integrate redundant calculation operators(operator fusion), and OPE can reasonably split the operators according to the hardware storage characteristics(operator split). These two modules can improve the inference efficiency from the two perspectives of fusion computing and adjusting the data storage structure. The SPE plays a very important role, and it is the key to the model's shift from string computing to parallel computing. Taking into account the differences in parallel capabilities between different side-end hardware devices, it has the characteristics of hardware adaptive partitioning, that is, it provides an efficient parallel solution based on the Parallel capability of hardware.

% \hwsay{We cannot call this part as image partitioner as we want to claim \sysname can work for not only CNNs, but also other types of DNNs.}

% \para{IP} 
% preprocesses the raw input, i.e., the image, before feeding it to Coordinator. After fetching the image data from the memory pool (EMPG), the IP module partitions the image according to the computation attributes of the beginning operator. \sysname supports both single-dimension and multi-dimension partition of images. For example, if the beginning operator is a depthwise separable convolution (i.e. input channel and output channel are the same, and both are equal to $1$ or $3$), then IP partitions the image by columns or rows according to the degree of parallelism. If the beginning operator is standard $3\times3$ (i.e. the input channel and the output channel are not consistent), then IP conducts channel-based partition to achieve good parallelism.

% \para{PP} 
% conducts parameter (i.e. feature map) \hwsay{`Feature map' is not the same with `parameter'. `Parameter' is the model, and `feature map' is the output tensor for each operator. For example, convolution  kernel is `parameter', not `feature map'.} preprocessing for the inference model. As described in \S\ref{sec-op-reshape}, the computation operators will be fused/split for \hapstrategy strategy. Correspondingly, PP concatenates or splits the feature maps to match the partitioned model.  

% \para{MG}
% is the main module for inference. It holds the operator library, which possesses a variety of computation operators. These operators are manipulated by the two functional sub-modules in MG, namely, Model Partitioner (MP) \hwsay{Model Partitioner is confusing with Parameter Partitioner.} and Dataflow Restructurer (DR), which conducts the \hapstrategy strategy (described in~\S\ref{sec-ha-strategy}) and the \idrstrategy strategy (described in~\S\ref{sec-dr-strategy}) respectively.

% \para{RD}
% is mainly responsible to generate the profiling report for the model inference on the hardware platform as an extended part of \sysname. The profiled metrics include memory cost, computing resource cost, and the time cost (including both the total time cost and the individual time cost of each module). The reports can help to identify the bottleneck of the model inference and also serve as useful guidance for engineers to further optimize the model structure.

% \hwsay{What is the relationship between these modules and the following sections? They are seldom mentioned in the following sections?}

%and model researchers can quickly adjust the model structure to meet the actual required performance indicators based on the deployment report. Thereby, the RD module can compress the entire model deployment cycle.

%As we all know, the in-depth model structure and large-scale parameters can better obtain image texture information, thereby obtaining more accurate predictions. Because of this, model researchers usually cannot accurately grasp the relationship between model scale and side-end hardware resources. Neural Architecture Search (NAS) technology can provide reference models for hardware characteristics, but it often requires a large number of iterative processes and high time costs. The deployment report generated by RD can accurately and directly locate the bottleneck point of the model, and model researchers can quickly adjust the model structure to meet the actual required performance indicators based on the deployment report. Thereby, the RD module can compress the entire model deployment cycle.



% The inference task is usually not implemented offline or in a single part, and requires coordination of multiple parties. Therefore, we designed the complete architecture of \sysname (as shown in Figure \ref{arch}), which includes Data Plane (DP), Master Device (MD) and Slave Device (SD).
% \textbf{SD logic.} We design SD to be responsible for image data acquisition tasks, which have high-speed and real-time image capture capabilities. In order to make the image-data reach the preprocessing equipment (MD) quickly, we adopt Low-Voltage Differential Signaling (LVDS) technology for communication, which uses very low voltage swing to transmit data at high speed. Taking into account the problem of congestion during transmission and at the end, we adopted an efficient queue and efficient Memory Pool to alleviate it.

% \textbf{MD logic.} On the MD side, it mainly includes five components, namely Image Distributor (ID), Parameter Distributor (PD), Preprocessor (PP), Coordinator and Efficient Memory Pool Group (EMPG). ID is responsible for dividing the image-data transmitted by DP according to the hardware parallel capability. PD is responsible for dividing computing tasks and parameters according to hardware parallel processing capabilities. PP is mainly responsible for two tasks. One is that in order to enable the inference model(in the SD) to obtain high-quality images-data, it is necessary to perform a series of enhancement tasks. The second is to resize the image to meets the size required by the inference model. EMPG contains multiple types of storage media, their functions are independent of each other, and can meet the read and write operations of multiple data types. Coordinator is responsible for assisting the connection between the modules and the communication with peripherals. Considering the scalability, between MD and SD, we reserve a variety of communication methods to meet the needs of different hardware.

% \textbf{SD logic.} In SD, there are mainly five components, namely Image Distributor (ID), Parameter Distributor (PD), Model Generator (MG), Coordinator and Efficient Memory Pool Group (EMPG). Before the start of each inference, ID will load the current latest or preprocessed image in the historical sequence as required. After that, it will be divided according to parallelism and model attributes. Taking SkyNet and MobileNet models as examples, the first layer of the Skynet model is deepth-conv$3\times3$ layer, and the input channel and output channel are both 3. If the parallelism is 8, we need divide by row or column. On the contrary, the first layer of the MobileNet model is a standard $3\times3$ convolution, with input channels of 3 and output channels of 32. If the parallelism is 8, we can directly divide the data according to the channel to avoid the data fusion step.
% The PD is responsible for dividing the parameters according to the size of the parameters and the hardware storage characteristics. In the actual workflow, the parameters of each layer of the model are different and the model layers need to be combined flexibly before calculation \footnote{Different combinations correspond to different parameter divisions.For example, operator fusion needs to divide the parameters evenly and recombine them, and operator splitting needs to divide the parameters evenly after splitting them.}. Many factors need to be considered comprehensively, so we use Coordinator to assist in management and ensure accurate alignment of parameters and models. In addition, Coordinator also uses a variety of efficient skills. For example, Assist PD to increase the overlap between parameters communication time and model calculation time through Pipeline, and reduce hiding time. MG is mainly responsible for generating the inference model of the target hardware, which is the core module in SD. Taking into account the differences between different hardware platforms, it needs to divide the model according to heuristic algorithms. Before model combination, it also needs to perceive the model-layer context and adopt fine-grained data reconstruction to ensure the overall efficiency of reasoning. EMPG uniformly manages data read, write and reuse. In the inference process, there will be a lot of temporary data, such as the jump connection of the model needs to consider additional data processing and so on.



\subsection{Efficient Memory Pool Group}
During the inference process, the frequent swap of feature map data (with variable sizes) can lead to memory fragmentation problems. To mitigate the fragmentation and better explore the cache benefit, we develop an efficient \emph{memory reuse mechanism} in EMPG. The reuse mechanism follows the typical producer-consumer model. Before the launch of the inference process, EMPG prepares in advance a pool of memory chunks, with typical model layer sizes. While allocating memory for a fresh model layer, EMPG first checks the available memory chunks with the same size (or even larger size), then allocates a suitable chunk to hold the model layer. Meanwhile, the chunk is marked as \emph{in-use}. When the lifetime of the model layer is terminated, the chunk is marked again as \emph{available} and recycled in the memory pool, so that EMPG can use it for the other incoming model layers. Besides, for very small data, EMPG will also do batching with them and fit them into one memory chunk. In this way, the fragmentation is further reduced and data locality is much preserved. 


\subsection{Operator Elastic Combination}
\label{sec-op-reshape}

A neural network (NN) model is typically represented as a computation graph in existing NN frameworks like PyTorch~\cite{pytorch} or TensorFlow~\cite{abadi2016tensorflow}.With reference to the computation graph, it is straightforward to generate a complete but unoptimized inference code using existing operator library. 
However, the unoptimized code involves redundant or inefficient memory access, leading to poor performance. 
Operator fusion, which is a widely used optimization technique, can significantly reduce the redundant memory access, but still misses many optimization opportunities.
Targeting at this, \sysname proposes OEC, including operator linking and split, to further improve memory efficiency. 

\para{Operator linking.}
Operator fusion are commonly used optimizations in existing NN frameworks.
Typical operator fusion mainly fuses element-wise operators with their adjacent operators, so that the extra memory read and write between operators can be eliminated thus improving the memory efficiency.
Besides operator fusion, IDR gives \sysname{} the opportunities to further reduce memory overhead, which we call {\it operator linking}.

As shown in \Cref{opfusion}~(a), fusing operators {\tt Conv1x1}, {\tt Bn}, {\tt Bias} and {\tt Relu} into one operator {\tt CBR} is a typical optimization. 
However, simply fusing operator {\tt CBR} and {\tt AvgPooling} will usually not get better memory performance due to the complex dataflow on the input feature map of {\tt AvgPooling} (a 2-D sliding window).
As shown in \Cref{fig:link}, the dataflow of {\tt conv}'s output mismatches with the dataflow required by {\tt AvgPooling}'s input, leading to extra data shuffle overhead even when these two operators are fused.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.6\linewidth]{./fig/link.pdf}
	\caption{Dataflow mismatch between {\tt conv}'s output and {\tt AvgPooling}'s input.}
	\label{fig:link}
	\vspace{-0.2cm}
\end{figure}

Based on IDR, \sysname{} is able to reorganize the dataflow.
As shown in \Cref{opfusion}~(b), operator {\tt CBR} and operator {\tt AvgPooling} will be marked as linkable operators in OEC.
In IDR, the feature map dataflow of linked operator will be reorganized to eliminate the data shuffle overhead, and the detail will be illustrated in \S\ref{sec-dr-strategy}.

\input{algo/link}

\Cref{algo:link} shows the algorithm of performing fusion and linking on a given computation graph in \sysname{}.
\sysname{} will first try to fuse all the fusable operators, which is similar with existing NN frameworks.
Then for the unfusable operators, \sysname{} will link them if the size of their parameters are less than a certain size $threshold$, which is set as the L2 memory size in \sysname{}. 
The dataflow of linked operators will be optimized in IDR.


% {
% However, as mentioned before, \sysname{} 
% Thus, we provide an approach, called OEC, which can {\it logically} fuse and split operators by reorganizing the model parameters which can also achieve similar optimization effect.
% We call the operator fusion and split in OEC are logical because we do not actually generate the fused and splitted operators, but using existing operators with the reorganization of model parameters and the data restructuring of IDR.
% In this subsection, we will illustrate the different types of logical fusion and split, how to process model parameters to support such logical transformations, and how to choose a memory efficient logical transformation by considering the constrained resources on edge devices.
% How to apply the logical transformations to improve the inference performance will be illustrated in \S\ref{sec-dr-strategy}.
% }


% \para{IDR-based Fusion}
% Conv Bn Bias Relu (everyone does that)

% + fuse Maxpooling (Our advantage)

% CBRA-0 + CBRA-1 (b,c,d)
% \para{Memory-Aware Split}
% % \hwsay{`Reshape' is not a good name as there is an operator called `reshape' in NN. Reschedule?}

% % Given a neural network (NN) model trained from a typical ML framework (e.g. Tensorflow, Pytorch, etc.), we usually need to use Onnx\cite{onnx} or other tools to perform high-level computational graph representation. 

% %Targeting at the parameters in the inference model, \sysname relies on OEC to elastically fuse/split them for fast computation and memory efficiency. 

% \hw{Operator fusion and splitting are commonly used optimizations in existing NN frameworks on GPU to improve the memory efficiency by using the fused or splitted operators provided by NN libraries like cuDNN~\tocite{} or cuBLAS~\tocite{}. 
% However, such approach is not practical on edge devices as it requires a powerful NN library containing the implementation of different fused and splitted operators which usually does not exist on edge devices.
% Thus, we provide an approach, called OEC, which can {\it logically} fuse and split operators by reorganizing the model parameters which can also achieve similar optimization effect.
% We call the operator fusion and split in OEC are logical because we do not actually generate the fused and splitted operators, but using existing operators with the reorganization of model parameters and the data restructuring of IDR.
% In this subsection, we will illustrate the different types of logical fusion and split, how to process model parameters to support such logical transformations, and how to choose a memory efficient logical transformation by considering the constrained resources on edge devices.
% How to apply the logical transformations to improve the inference performance will be illustrated in \S\ref{sec-dr-strategy}.
% }

% \cred{Just as in existing ML training frameworks, like TensorFlow or Pytorch, a neural network (NN) model is typically represented as a computation graph.
% % \hw{A neural network (NN) model is typically represented as a computation graph in existing ML training frameworks, like TensorFlow or Pytorch.}
% % With reference to the high-level computational graph, 
% With reference to the computation graph, it is straightforward to generate a complete but unoptimized inference code using existing operator library. However, the unoptimized code involves redundant computation and is not memory-efficient. Targeting at this, \sysname relies on OEC to elastically fuse/split the model parameters for faster computation and memory efficiency. }
% \hw{to be removed}

% \sysname reshapes the operators to save computation/storage cost. The operator reshaping is executed by the Operator Elastic  Combination (OEC) component in MP.  


% Then, the unoptimized code will be handed over to the MG module, where the MP sub-module partitions the model and then the DR sub-module restructures the dataflow.


% MP relies on two main components, Operator Elastic  Combination (OEC) and Smart Parallel Execution (SPE) to refine the code for hardware-adaptive model partition. Besides, targeting these operators, DR also restructures the dataflow by modifying the writing order of parameters output by operators, so as to match it to the data access order of the subsequent operators.


% In order to achieve fast inference with economic memory cost, \sysname adopts a novel \emph{hardware-adaptive model partition} (HAP) strategy. The execution of HAP strategy relies on two main components, i.e. operator elastic combination (\S\ref{sec-oec}) and smart parallel execution (\S\ref{sec-spe}). 



% \hwsay{Give a concrete explanation for \Cref{opfusion}. For example, what does CBRA means? A fused operator of conv, bias, relu and maxpool. Explain how CBRA\_1 is splitted. What does HHF in the right part of \Cref{opfusion} mean? Further fusion?}


% \begin{itemize}[wide, labelwidth=!,nosep]
% \para{Operator Fusion.} OEC supports three main types of fusion, i.e parameter-level hierarchical fusion(PHF), hierarchical vertical fusion(HVF), and hierarchical horizontal fusion(HHF). PHF aggregates the parameters of the original operators and reuse them in the inference computation, so as to reduce redundant computation. HVF and HHF do not aggregate the original parameters. HVF fuses multiple operators (which operate on the same feature maps) for temporal data locality. HHF fuses same-type operators to improve parallelism. We use three examples to explain them separately.

% \begin{itemize}[leftmargin=*]
%     \item Equation~\ref{f1}-\ref{f3} give an example of PHF. The original operators (Equation~\ref{f1}-\ref{f2}) include convolution computation (Equation~\ref{f1}) and batch normalization (Equation~\ref{f2}). PHF fuses the two operators and yield a new operator (Equation~\ref{f3}). In Equation~\ref{f3}, $\frac{\gamma w}{\sqrt{\sigma^{2}+\varepsilon}}$ and $\beta + \frac{\gamma (B - \mu)}{\sqrt{\sigma^{2}+\varepsilon}}$ become the new parameters for the fused operator, which can be pre-computed to reduce the redundant computation of the original operators (Equation~\ref{f1}-\ref{f2}). 
%     \hw{In this case, we need to preprocess the parameters, which will be later used by IDR.}
%     \begin{equation} 
% \label{f1}
% y(x_{i}) = Wx_{i} + B
% \end{equation}
% \begin{equation}
% \label{f2}
% BN(y) = \gamma \frac{y-\mu}{\sqrt{\sigma^{2}+\varepsilon}} + \beta
% \end{equation}
% \begin{equation}
% \label{f3}
% F(x_{i}) = \frac{\gamma W}{\sqrt{\sigma^{2}+\varepsilon}}x_{i} + (\beta + \frac{\gamma (B - \mu)}{\sqrt{\sigma^{2}+\varepsilon}})
% \end{equation} 
%     %\footnote{Among them, $\mu$ and $\sigma^{2}$ are the parameters trained in the BN layer, which are $\mu=\frac{1}{m} \sum_{i=1}^{m} x_{i}$ and $\sigma^{2}=\frac{1}{m} \sum_{i=1}^{m}\left(x_{i}-\mu\right)^{2}$ respectively.$\gamma$ and $\beta$ are the trained scaling factors, and $\varepsilon$ is a constant.}.
%     \item Equation~\ref{hvf-f1}-\ref{hvf-f3} give an example of HVF. The original operators (Equation~\ref{hvf-f1}-\ref{hvf-f2}) include convolution computation (Equation~\ref{hvf-f1}) and relu computation (Equation~\ref{hvf-f2}) \hw{I suggest use {\tt conv-maxpool} instead of {\tt conv-relu} since 1) the former one is more complex and not a widely used fusion; 2) we can tell a more complete story along with IDR (fig 5).}. HVF fuses them and yield a new operator (Equation~\ref{hvf-f3}). Unlike PHF, the fused operator of HVF does not have new parameters, i.e. it still uses the parameters from the original operator (Equation~\ref{hvf-f1})~\footnote{The Relu operator does not have parameters.}. However, the fused operator enjoys better temporal locality and avoids unnecessary data accesses. With the original operators, each feature map element $x_i$ needs to be accessed twice. The inference engine first computes the convolution for all feature map elements $x_i$ and then continues to compute the relu value for them. These feature map elements need to be swapped in and out. In contrast, with the fused operator, each $x_i$ is only accessed once and the inference engine completes both the convolution and the relu computation for it. After that, $x_i$ is swapped out and no longer needed.
% \begin{equation} 
% \label{hvf-f1}
% y(a_{i,j}) = Wa_{i,j} + B
% \end{equation}
% \begin{equation} 
% \label{hvf-f2}
% Max-Pooling(a_{i,j},a_{i,j+1},a_{i+1,j},a_{i+1,j+1}) = \max\{a_{i,j},a_{i,j+1},a_{i+1,j},a_{i+1,j+1}\}
% \end{equation}
% \begin{equation} 
% \label{hvf-f3}
% Max-Pooling(y) = Relu(Wx_i+B)
% \end{equation}

% \item Equation~\ref{hhf-f1}-\ref{hhf-f3} give an example of HHF. The original operators (Equation~\ref{hhf-f1}-\ref{hhf-f2}) both conduct convolution computation towards the same feature map. Instead of computing them separately, HHF first concatenates the parameters of these two operators and computes them as one operator (Equation~\ref{hhf-f3}), which achieves higher parallelism.
% \hw{Parameter preprocess}



% \begin{equation} 
% \label{hhf-f1}
% y_{1}(x_{i}) = W_{1}x_{i} + B_{1}
% \end{equation}
% \begin{equation} 
% \label{hhf-f2}
% y_{2}(x_{i}) = W_{2}x_{i} + B_{2}
% \end{equation}
% \begin{equation} 
% \label{hhf-f3}
% y_{0}(x_{i}) = Concat(W_1, W_2) x_i + Concat(B_1, B_2)
% \end{equation}

% \end{itemize}
% \hwsay{What is the difference between PHF, HVF and HHF? What are these three words mean? Give a precise definition.}


% four operators (i.e. conv, bias, relu and maxpool) into two fused operators named CBRA-0 and CBRA-1, which can save redundant computation and be executed faster. Considering the large size of CBRA-1, which fails to fit into the L2 cache, OEC continues to split CBRA-1 into finer-grained ones (i.e. CBRA-10 and CBRA-11) and opportunistically fuses CBRA-0 and CBRA-10 for better performance. 






% Equation~\ref{??}-\ref{??} and Equation~\ref{??}-\ref{??} (\rv{add example formula, may be put in appendix}) illustrate examples of HHF and HVF respectively. 
% HVF fuses the conv-layer, bias-layer, and relu-layer into one layer. Such fusion avoids a large amount of memory swapping in and out, thereby improving the efficiency of reasoning. HHF fuses conv-layers with the same attributes to avoid redundant computing resource cost caused by repeated computation, and it also saves memory space.





% OEC also supports dimension-based operator split.


% To handle large-sized operator parameters and fit them into L2 cache, OEC splits the parameters according to a specific dimension. 


\para{Dimension-based memory-aware operator split.}
As we mentioned before, parameters are stored in L2 memory, which is private storage for each DSP unit, meaning that the parameters have to be split into different L2 memory.
Moreover, if the parameter size is too large to fit into L2 memory, it will lead to significant performance loss.
OEC uses dimension-based memory-aware operator split to address these problems.

OEC performs two-stage operator split based on HAP.
At the first stage, OEC splits the parameters into $n$ parts, where $n$ is the number of DSPs, and each DSP unit responds for the computation corresponding to the parameters it holds.
Note that we do not need to split the feature maps for each DSP unit as feature maps are store on shared memory which is visible for all DSPs.
At the second stage, if the size of each DSP unit's parameter is larger than L2 memory, it will be further split into multiple partitions to fit the L2 memory.

At each stage, the OEC follows a certain priority for each dimension when performing parameter splitting, to guarantee that minimum computation overhead is introduced after splitting.
Taking the popular CNN model as an example, which have four dimensions for parameters, i.e., output channel ($K$), input channel ($C$), kernel height ($R$), and kernel width ($S$).
Splitting at $K$ dimension will not introduce any extra computation, while splitting at other three dimensions requires additional reduction operation to aggregate the results on these dimensions, which introduces extra computation overhead.
Thus, OEC will first try to split the parameters at $K$ dimension, and then $C$, $R$ and $S$ if only splitting $K$ dimension is not enough to fit the parameter in L2 memory. 
% \hw{Do we have any example of splitting along other dimensions?}

% support three main types of operator split, i.e. (output)-channel-based split (CBS), height-based split (HBS), and width-based split (WBS), which split the parameters. 
% OEC does not split parameters based on input channels: If OEC split the operator parameters based on the input channels, it would require OEC to conduct extra reduction operation to aggregate the output feature maps output from each split operators, which adds much complexity and overheads.

%\hwsay{These three types of split are CNN specific. May be using dimension-aware split? Dimension-aware comes from two aspects: 1. Reduction \& non-reduction dimension, like C or H; 2. Inner and outer dimension, like H and W.} \rv{Why output channel-partition rather than input-channel-partition? Input channel-partition will lead to reduction after each operator.}
% For edge devices with multi-level memory, it is usually necessary to  consider hardware computing and storage capabilities. Therefore, we need to split the computation of some operators to adapt to specific resource constraints. 

Equation~\ref{f4} gives an example of output-channel-based splitting. Since the large-sized parameters ($W$ and $B$) can not be put into the L2 memory, OEC performs fine-grained split of the operator:
$W$ is split into $W_1$ and $W_2$, and $B$ is split into $B_1$ and $B_2$. 
After that, parameters can be distributed into the L2 memory of two different DSP units. 
Equation~$y_0$ and $y_1$ can be jointly executed on two DSP units in parallel, or on one DSP unit one by one.
The output $y_{1}(x_{i})$ and $y_{2}(x_{i})$ are automatically joined together using IDR, without performing any data layout transformation operators. 
Other types of splitting work in a similar way.
\begin{align} 
\begin{aligned}
\label{f4}
y(x_{i}) &= Wx_{i} + B \\
&\Downarrow \\
y_{1}(x_{i}) &= W_{1}x_{i} + B_{1} \\
y_{2}(x_{i}) &= W_{2}x_{i} + B_{2}
\end{aligned}
\end{align}
% \begin{equation} 
% \label{f7}
% y_{0}(x_{i}) = Concat(y_{1}(x_{i}), y_{2}(x_{i}))
% \end{equation}

%Besides CBS, HBS and WBS comprehensively consider the relationship between feature map size and storage space. Specifically, when the size of the feature map exceeds the storage area limit, HBS and WBS will split the feature degrees according to the remaining space of the current storage area, and the feature maps are calculated in batches, which can further improve resource reuse degree and inference efficiency.
% \end{itemize}

%In general, operator fusion aims to reduce redundant computation, and is conducted before executing the \hapstrategy strategy (described in \S\ref{sec-ha-strategy}). While executing the \hapstrategy strategy, \sysname can encounter situations where the operators cannot fit into the high-level memory~\footnote{Although the operator's weight parameter size tend to be far less than the feature map size \hwsay{may not be true}, it can also fail to fit into the L2 cache of one single DSP unit, and needs operator split to distribute the memory cost across multiple DSP units.}. In that case, the large-sized operator will be split into finer-grained ones (e.g. Equation~\ref{f4}-\ref{f7}), so that they can fit into the high-level L2 memory of multiple DSP units and be jointly executed. 



\para{Example optimization process.} 
Equipped with the fusion, link and split capality of OEC, a concrete user case of operator optimization is illustrated in Figure~\ref{opfusion}.
\begin{figure}[h]
	\centering
	\includegraphics[width=0.48\textwidth]{./fig/opfusion.pdf}
	\caption{Illustration of Operator Elastic Combination.}
	\label{opfusion}
	\vspace{-0.5cm}
\end{figure}


% \subsubsection{Operator Elastic Combination (OEC)}
% \label{sec-oec}
% As shown in Figure 
\Cref{opfusion} gives an example of how OEC optimizes a part of the computation graph of MobileNet~\cite{howard2017mobilenets}. 
OEC first performs operator fusion on operator {\tt Conv1x1} (convolution), {\tt Bn} (batch normalization), {\tt Bias}, and {\tt Relu}, and generates a fused operator {\tt CBR}, then links {\tt CBR} and {\tt AvgPooling} together to form the operator {\tt CBRA}.
Operator {\tt CBRA} will be first split into eight partition to fit each DSP unit's L2 memory.
Considering that the parameter size of each partition ($1024 \times 1024 \times 1 \times 1 \times 4 \text{B} / 8 = 512 \text{KB}$ for convolution kernel, and $1024 \times 7 \times 7 \times 4 \text{B} / 8 = 24.5 \text{KB}$ for bias) is larger than L2 memory size ($512 \text{KB}$), thus it will be further split into two partitions and executed one by one on each DSP unit.

% and Max-Pooling) by HVF, yielding CBRA-0 and CBRA-1. Then, since CBRA-1 is too large to fit into L2 cache, \sysname split CBRA-1 into CBRA-10 and CBRA-11, and CBRA-11 is able to fit into the L2 cache of one DSP core, whereas CBRA-0 and CBRA-10 are fused again by HHF to fit into the L2 cache of the other DSP core.


\subsection{Operator Partition} 
\label{sec-ha-strategy}

% \subsubsection{Smart Parallel Execution (SPE)}
% \label{sec-spe}

\begin{algorithm}[!htbp]
\small
\makeatletter
\NewDocumentCommand{\LeftComment}{s m}{%
  \Statex \IfBooleanF{#1}{\hspace*{\ALG@thistlm}}\(\triangleright\) #2}
\makeatother

\algdef{SE}[EVENT]{Event}{EndEvent}[1]{\textbf{upon}\ \textsc{\small #1}\ \algorithmicdo}{\algorithmicend\ \textbf{event}}%
\algtext*{EndEvent}
\caption{Operator Partition}
\label{algo-spe}
\hspace*{\algorithmicindent} \textbf{Input}: 

\hspace*{\algorithmicindent}
\emph{\textbf{inH: }}{The input height of the feature map.}

\hspace*{\algorithmicindent}
\emph{\textbf{inW: }}{The input width of the feature map.}

\hspace*{\algorithmicindent}
\emph{\textbf{outC: }}{The output channel number of the feature map, i.e. the \hspace*{\algorithmicindent} number of kernels in this operator.}

\hspace*{\algorithmicindent}
\emph{\textbf{K}}\textbf{[$1\dots outC$]:} {The list of kernels}

\hspace*{\algorithmicindent} 
\emph{\textbf{F}}\textbf{[$1\dots inH$] [$1\dots inW$] [$1\dots inC$]: }{The input feature map, size \hspace*{\algorithmicindent}of $inH\times inW\times inC$.}

\hspace*{\algorithmicindent} \emph{\textbf{P: }}{The expected parallelism degree, i.e. the number of DSP \hspace*{\algorithmicindent} units available on the edge device.}

  \begin{algorithmic}[1]
  \Event{\text{receiving} (\emph{K, F})}
      \hspace*{\algorithmicindent} \LeftComment{While receiving a feature map $F$ and the target operator (kernels) $K$, we output a partitioned $scheme$. We assume $P$ is global constant}
    \State $scheme=$ \textsc{fmp-algo}($K, F, P$)
    \State Forward $scheme$ to Inference Engine
  \EndEvent
  
 
     \Function{fmp-algo}{$K, F, P$}
        \LeftComment{$scheme$ is encoded as a dictionary, with key as the } \LeftComment{core-id and value as the partitioned operators and} \LeftComment{feature map (fmp) assigned to this core }
        \For{$i$ $\gets$1 to $P$}
         \Comment{Initialization of $scheme$}
            \State $scheme$[$i$]=$\{kernel:\{\}, fmp:\{\}\}$
           
        \EndFor
        
        \LeftComment{Partition by output channel $outC$}
        \State $sliceByC=\lfloor outC/P \rfloor$
        \For{$i\gets$1 to $P$}
        \LeftComment{{\small $K$[$k_1:k_2$]  represents a slice in $K$, ranging from $k_1$ to $k_2$}}
            \State $k_1=\emph{sliceByC}\times(i-1)+1$
            \State $k_2=k_1+sliceByC$
            \State $scheme$[$i$][\emph{kernel}].append($K$[$k_1$:$k_2$])
            \State
            $scheme$[$i$][\emph{fmp}].append($F$)
        \EndFor
        
        \State $restC=sliceByC\times P+1$ 
        \LeftComment{Partition by input height $inH$}
        \State $K'=\emph{K}$[\emph{restC}:\emph{outC}]
        \State $sliceByH=\lfloor inH/Pn \rfloor$
        \For{$i\gets$1 to $P$}
            \State $h_1=\emph{sliceByH}\times(i-1)+1$
            \State $h_2=h_1+sliceByH$
            \State $scheme$[$i$][\emph{kernel}].append($K'$)
            \State
            $scheme$[$i$][\emph{fmp}].append($F$[$h_1$:$h_2$][:][:])
        \EndFor
        
        \State $\emph{restH}=\emph{sliceByH}\times P+1$ 
        \LeftComment{Partition by input width $inW$}

        \State $\emph{sliceByW}=\lfloor inW/P \rfloor$
        \State $F'=F[restH:outH][:][:]$
        \For{$i\gets$1 to $P$}
            \State $w_1=\emph{sliceByW}\times(i-1)+1$
            \State $w_2=w_1+\emph{sliceByW}$
            \State $scheme$[$i$][\emph{kernel}].append($K'$)
            \State
            $scheme$[$i$][\emph{fmp}].append($F'$[:][$w_1$:$w_2$][:])
        \EndFor
        
        
        \LeftComment{Randomly assign the remaining feature map}
        \State $\emph{restW}=\emph{sliceByW}\times P+1$
        \For{$i$ $\gets$ $restW$ to $inW$}
            
            \State $\emph{F''}=$$F$[:][$i$][:] \Comment{Pick the $i$th column of $F$}
            \State $r$=\textsc{rand}()$\%W$
            \Comment{Assign to a random DSP unit}
            \State  $scheme$[$r$][\emph{fmp}].append($F''$) 
            \State $scheme$[$r$][\emph{kernel}].append($K'$)
        \EndFor
    \State \Return $scheme$
     \EndFunction
  \end{algorithmic}
\end{algorithm}

% \hwsay{Relationsip between HAP and operator split? Operator split indicates how an operator can be splitted, and HAP illustrates how a model should be partitioned to achieve higher performance given a specific hardware. Am I right?}


Given OEC's capability of fusing/splitting/linking operators, \sysname circumvents the memory constraints and places all parameters into L2 memory. Still, it is insufficient for high parallelism, so \sysname employs FMP to partition the feature maps based on HAP and share the inference workload across multiple DSP units.



% the SPE component aims to conduct efficient parallel execution of these operators according to the number of available DSP units, as well as increase the overlap between parameter communication and inference computation. 

% The main idea of \hapstrategy is to partition the feature maps across multiple computation units (DSP cores), so that they can jointly undertake the inference workload with high parallelism. During the partition, there are two main concerning issues. First, \hapstrategy aims to achieve load balance across DSP cores and avoid straggler effect. To do that, the feature maps are partitioned by its different dimensions (e.g. height, width, channel, etc.). Each DSP core takes charge of one partitioned feature map and the corresponding operators for inference. Second, whereas the feature map is completely held by the main memory, \hapstrategy aims to place the operator parameters (e.g. weights) into high-level memory (L2 cache) for efficiency. When \hapstrategy encounters some large-sized operator, it relies on OEC to split the operator into multiple finer-grained ones (\S\ref{sec-op-reshape}) and distribute them into the L2 cache of multiple DSP cores. 

Algorithm~\ref{algo-spe} exemplifies the feature map partition for typical CNN models. For simplicity, the algorithm assumes that the operators have already been splitted by OEC, thus all the parameters can be fit into L2 memory.
When the operator parameters (e.g. the CNN model has very large-sized kernels) cannot fit into the L2 memory, FMP contacts OEC to split the operator parameters first, and then the feature map will be partitioned following the similar logic in Algorithm~\ref{algo-spe}.
Actually operator split in OEC shares similar algorithm with FMP as they are both based on HAP.

As shown in Algorithm~\ref{algo-spe}, FMP considers partitioning the feature map in three dimensions, namely, the input feature map height ($inH$), the input feature map width ($inW$), and the output feature map channel ($outC$). Here we omit the input-channel-based partition for simplicity since we need to perform extra reduction if we partition along input channel which will introduce computation overhead. Considering that the feature maps are stored in the shared memory with size of $4$ MB, which is far beyond the input channel size in typical CNN model, we usually do not have to partition along input channel. 

FMP prioritizes $outC$-based partition (line 7-13) due to its less complexity: FMP simply distributes the kernel parameters to different DSP units, and these kernel parameters will be placed into the L2 memory of DSP units. All DSP units can access the feature map located in the shared memory. On the other hand, $inH$-based scheme (line 14-21) and $inW$-based scheme (line 22-28) partition the remaining feature map after $outC$-based partition, and they usually require special handling of the boundary rows/columns. Only if the kernels cannot be evenly distributed across DSP units, FMP will seek further partition by $inH$/$inW$. If imbalance still exists after the triple partition, FMP will randomly assign the remaining feature map (workload) to different DSP units (line 29-34).
%\hw{Check line numbers. Done}

%Therefore, \hapstrategy first conducts $outC$-based partition. 

% Corresponding to the operator split, an input feature map is be partitioned in three dimensions, namely, the input feature map height (InH), the input feature map width (InW), and the output feature map channel (OutC). Partitioning according to InH or InW will result in a large number of padding operations and require fine-grained data splicing after the calculation. More importantly, this type of partitioning method requires each DSP unit to load all convolution kernel parameters, which will cost additional memory overheads. Conversely, partitioning through OutC can distribute the convolution kernel parameters more evenly, and data splicing is also more convenient. However, even OutC-based partition cannot fit the DSP unit resource constraints in common cases. In order to achieve efficient inference, SPE adopts a finer-grained way to partition. To be more specific, the SPE partition algorithm prioritizes the OutC-based partition, but also leverages the InH-based partition or InW-based partition when the OutC-based partition cannot achieve balanced distribution. 

% By such a hierarchical partition, \sysname is able to maximize the load balance among different computation units. Equipped with SPE, \sysname is able to partition most typical operators, including depthwise separable conv $3\times3$ operator, depthwise separable conv $1\times1$ operator, or standard convolution operator, and evenly distribute the computation workload among the computation units.

% in LNN can be evenly distributed after Case 0 and/or Case 1. the depth-separable $1\times1$ or standard convolution, InC != OutC, but we can achieve partition optimization based on partition schemes similar to Case0 and Case1.



% During the execution of SPE, the operator are first categorized into four cases by making two comparison, i.e. the comparison between the number of input map channels (InC) and the number of output map channels (outC), and the comparison between the number of output map channels (OutC) and the number of DSP units (Pn).

% \begin{itemize}
%     \item Case 0: $(InC == OutC) \ \&\&\  (OutC \geq Pn)$;
%     \item Case 1: $(InC == OutC \ \&\&\ OutC \textless Pn)$;
%     \item Case 2: $(InC != OutC \ \&\&\ OutC \geq Pn)$;
%     \item Case 3: $(InC != OutC \ \&\&\ OutC \textless Pn)$.
% \end{itemize}
 

% For Case 0, SPE will first partition according to OutC. Failing to achieve evenly distribution, SPE will continue to partition according to InH or InW, which is similar to Case 1. 

% For Case 1, the number of output channels (OutC) is less than the number of DSP computation units (Pn), so SPE partitions the model according to InH. The algorithm comes to the end if the model has been evenly distributed after the InH-based partition. Otherwise, SPE continues to partition according to InW. If the algorithm still fails to achieve evenly distribution afer InW-based partition, the remaining part will be randomly distributed. 

% Case 0 and Case 1 are mainly designed for the partition of depth-separable $3\times3$ operator, which has equal input channel and output channel. When partitioning the depth-separable $1\times1$ or standard convolution operator, which have different input channel number and output channel number (i.e. InC $\neq$ outC), we use slightly different partition methods, 




% Hardware-Adaptive Model Partition
% 1. Elastic Combination Combination = Fusion + Operator Split
% 2. Parallel Execution

% Dataflow Rescheduling(Restructuring)

%\rv{Rewrite the algo with comments}







% \begin{algorithm}[t]
% \begin{algorithmic}
% 	\caption{Smart Parallel Execution Algorithm}
% 	\label{main}
% 	\KwIn{ \\ $NPO$ : Non-Parallel elastic combination operators.
% 	       \\ $ParasSet$ : FmH, FmW, FmC, KSize, etc.
% 	       \\$Pn $ = Parallelism degree
% 	}
% 	\KwOut{ \\  $PO$ : Parallel Elastic Combination Operators.
% 	        \\  $ParasSet$ : FmH, FmW, FmC, Kernel Size, etc.
% 	}
% 	\SetKwFunction{FMain}{Xenos\_SPE\_Main}
% 	\SetKwFunction{SPE}{SPE\_Partitioner}
% 	\SetKwProg{Main}{}{}{}
% 	\SetKwProg{Fn}{function}{}{}
	
% 	\Main{\FMain{}}{
% 	    \ForAll{$e \in NPO$}{
% 	     \texttt{$PO, ParasSet$}= \texttt{SPE\_Partitioner}($e.OutC, e.InH,$ \\$e.InW, Pn$)\textbf{;}\\
% 	     \State Transmit $PO, ParasSet$ to LNN Inference Engine
% 	     }
% 	    \EndFor
	    
        
% 	} 
% 	\Main{\SPE{OutC, InH, InW, Pn}}
% 	{
% 	\tcp{\small Out-Channel partition at the highest priority}
% 		\If{OutC \geq Pn}
% 		{
% 		    {\rm Partition by} $OutC$\textbf{;}\\
% 		    \If{(OutC \% Pn == 0)}
% 		    {
% 		        \rm{}
% 			    \textbf{return $PO$, $ParasSet$;}
% 			}
% 		}
% 	    \If{($InH$ \% Pn   == 0)}
% 	    {
% 	        \rm{}
% 	    	\textbf{return $PO$, $ParasSet$;}
% 	    }
%         {\rm Partition by} $InW$\textbf{;}\\

%         \If{($InW$ \% Pn == 0)}
%         {
%             \rm{}
%             \textbf{return $PO$, $ParasSet$;}
%         }
%         \Else
%         {
%             \rm{Randomly distributed by} $InW$;\\
%             \textbf{return $PO$, $ParasSet$;}
%         }
% 	}
% \end{algorithmic}
% \end{algorithm}
% \begin{algorithm}[h]
% 	\caption{Fixed Partitioner Algorithm}
% 	\label{Fixed}
	
% 	\KwIn{ \\ $NPO$ : Non-Parallel elastic combination operators.
% 	       \\ $Paras\_set$ : fm\_h, fm\_w, fm\_c, k\_size, etc.
% 	}
% 	\KwOut{ \\  $PO$ : Parallel Elastic Combination Operators.
% 	        \\  $Paras\_set$ : pfm\_h, pfm\_w, pfm\_c, k\_size, etc.
% 	}

% 	\SetKwProg{Main}{}{}{}
	

% \end{algorithm}

% \begin{algorithm}[h]
% 	\caption{Elastic Partitioner Algorithm}
% 	\label{Elastic}
% 	\KwIn{ \\ $NPO$ : Non-Parallel elastic combination operators.
% 	       \\ $Paras\_set$ : fm\_h, fm\_w, fm\_c, k\_size, etc.
% 	}
% 	\KwOut{ \\  $PO$ : Parallel Elastic Combination Operators.
% 	        \\  $Paras\_set$ : pfm\_h, pfm\_w, pfm\_c, k\_size, etc.
% 	}
% 	\SetKwFunction{Flexible}{Flexible\_Partitioner}
% 	\SetKwProg{Main}{}{}{}
% 	\SetKwProg{Fn}{function}{}{}
	
% 	\Main{\Flexible{}}
% 	{
%         \textbf{Case0:}\\
%         \If{(Pipeline by Out\_c or In\_c \textgreater PN)}
% 		{
% 		    Parallelism adjustment:\\
% 		    \If{(Pipeline by In\_h or Out\_h \textgreater PN)}
% 		    {
% 		        Adjust to In\_w or Out\_w level\textbf{;}\\
% 		        Same as Case0\textbf{...}\\
% 		        \textbf{Return $PO$, $Paras\_t$;}
% 		    }
% 		    \ElseIf{(Pipeline by In\_h or Out\_h \textless PN))}
%         	{
%         	    Partition by $In\_h$ or $Out\_h$ \textbf{then}\\
%         	    Unroll by $In\_h$ or $Out\_h$\textbf{;} \\
%         	    \textbf{Return $PO$, $Paras\_t$;}
%         	}
%             \ElseIf{(Pipeline by In\_h or Out\_h == PN))}
%         	{
%         	    Partition by $In\_h$ or $Out\_h$\textbf{;}\\
%         	    \textbf{Return $PO$, $Paras\_t$;}
%         	}
% 		}
% 		\textbf{Case1:}\\
% 		\ElseIf{(Pipeline by Out\_c or In\_c \textless PN))}
% 		{
% 		    Partition by $Out\_c$ or $In\_c$ \textbf{then}\\
% 		    Unroll by $Out\_c$ or $In\_c$\textbf{;} \\
% 		    \textbf{Return $PO$, $Paras\_t$;}
% 		}
% 		\textbf{Case2:}\\
% 	    \ElseIf{(Pipeline by Out\_c or In\_c == PN))}
% 		{
% 		    Partition by $Out\_c$ or $In\_c$\textbf{;}\\
% 		    \textbf{Return $PO$, $Paras\_t$;}
% 		}
% 	} 
% \end{algorithm}

\subsection{Inter-Operator Dataflow Restructuring}
\label{sec-dr-strategy}
% Main idea
% 1) matrix mul optim 
% 2) conv optim (padding)

%\hwsay{Difference with operator fusion?}

While \hapstrategy-based OEC and FMP enable high-parallel execution by reorganizing the parameters and feature maps,
% means of OEC's operator optimization and FMP's feature map partition, 
the dataflow during the execution is under-optimized and spoils the data locality.
To address that, \sysname employs IDR to conduct \emph{inter-operator dataflow restructuring}. 

\idrstrategy takes into account output/input sequence of adjacent operators. In other words, after one operator completes the inference computation, it should output the feature map to the shared memory in the desirable layout, so that the subsequent operators can read them with good data locality.  

% Therefore, we develop the fine-grained dataflow restructuring scheme based on inter-layer perception.
% \begin{figure}[t]
% 	\centering
% 	\subfigure[Restructure]{
% 		\label{1x1Restructure} 
% 		\includegraphics[width=1.6in]{./fig/1x1restructure.pdf}
% 	}
% 	\subfigure[FusionRestructure]{
% 	\label{fusionRestructure} 
% 	\includegraphics[width=1.6in]{./fig/fusionRestructure.pdf}


% 	}
% 	\caption{Inter-layer Aware Fine-grained Dataflow Restructuring}
% 	\label{Restructure} 
% 	\vspace{-0.3cm}
% \end{figure}


\begin{figure}[h]
	\centering
	\includegraphics[width=0.45\textwidth]{./fig/fusionRestructure.pdf}
	\caption{Dataflow restructuring}
	\label{fusionRestructure}
	\vspace{-0.3cm}
\end{figure}

We exemplify \idrstrategy with a linked operator ({\tt Conv1x1} + {\tt AvgPooling2x2}) in Figure~\ref{fusionRestructure}. The input feature map is generated by the previous operator which has 4 output channels, so the input feature map consists of four matrices (marked with different colors in Figure~\ref{fusionRestructure}). 

Without \idrstrategy optimization, the four matrices are placed into the memory one by one in a row-based manner, with the red one placed first, and the blue one placed last. However, during the inference computation, the fused operator needs to read $1\times1$ feature map from each matrix every time, and then computes the average on every $2\times2$ square after the convolution. As magnified on the right side of Figure~\ref{fusionRestructure}, the dataflow goes through the four matrices every time ({\tt Conv1x1} computation). On each matrix, it follows the zigzag pattern ({\tt AvgPooling} computation), leading to the restructured dataflow. Comparing the non-restructured and restructured pattern, the former one is oblivious to the data access, and each data access suffers from compulsory cache misses. By contrast, the latter one completely matches the data access pattern during the inference, so it maximizes the data locality and data can be fetched in much higher efficiency. 


To preserve the data locality, the previous operator is required to be aware of the data access pattern of the subsequent operator when it outputs the feature map. With such awareness, the inference engine can restruture the data layout following the access pattern, instead of simply outputting the matrices one by one. To attain this, IDR analyzes the adjacent operators linked by OEC, and pre-encodes the data access pattern of each operator in the optimized model. After the optimized model is fed into the inference engine, the inference engine gains the knowledge of the desirable feature map layout for each operator. During runtime, once an operator completes the inference computation and is about to output the feature map, the inference engine foresees the data access pattern of the subsequent operator and writes the feature map according to the pattern. Such a restructuring method involves data redundancy in standard convolution, since it replicates some parameters of the feature map to avoid the subsequent operator from looking back. However, the memory sacrifice proves to be worthwhile, because the performance benefit brought by the restructuring outweighes the additional memory cost and the inference workflow is effectively accelerated (shown in \S\ref{sec-exp-at}). 

% We use the typical combination of depthwise separable conv $3\times3$ layer and depthwise separable conv $1\times1$ layer in LNN as an example (as shown in Figure \ref{1x1Restructure}) to illustrate the rationale of dataflow restructuring. While the LNN Inference Engine is computing the depthwise separable conv $3\times3$ layer, the sequence of parameters is arranged in the order of  $W \times H \times C$ (i.e. first by row, and then by column, and finally by channel). After the inference, the parameters will be output (written) first by row, then by column, and finally by channel (refer to the non-restructured sequence in Figure~\ref{1x1Restructure} ). 
% However, while the LNN Inference Engine is computing the depthwise separable conv $1\times1$ layer, it needs to read the parameters in a channel-based way $C \times W \times H$ (refer to the restructured sequencer in Figure~\ref{1x1Restructure}). Without dataflow restructuring, the discontinuity of parameters spoils the spatial data locality and can break the cache mechanism of most side-end hardware, which eventually brings significant time cost. Such a situation is more severe for the operator fusion. If the depthwise separable conv $3\times3$ layer is followed by the depthwise separable conv $1\times1$ layer and AvgPooling fusion layer(as shown in Figure \ref{fusionRestructure}), then the data access sequence is not simply swapping the order of $W$, $H$ and $C$. In such a case, the dataflow restructuring becomes more complex considering the data access sequence of the fusion layer. For instance, if the stride parameter of AvgPooling is 2 (as shown in the case of Figure~\ref{fusionRestructure}), The data should be restructed according to $C \times W_{i} \times H_{j}$, $C \times W_{i+1} \times H_{j}$, $C \times W_{i} \times H_{j+1}$, $C \times W_{i+1} \times H_{j+1}$.


% For the sake of better locality, the inference computation of the previous layer is required to be aware of the data access pattern of the following inference computation behind it. In our example, the inference computation of the depthwise separable conv $3\times3$ layer should perceive the data access pattern of the computing task of the following depthwise separable conv $1\times1$ layer. To attain this, our LNN Inference Engine has tracked and pre-encoded the data access pattern of each layer before the inference starts. After computing one layer of inference, the LNN Inference Engine automatically checks the data access pattern of the next layer and writes the output parameters according to the pattern. Such a restructuring method involves data redundancy in standard convolution, since it replicates some parameters output from the previous layer to avoid the operators from looking back. 
% %The dataflow restructuring without optimization will cost more memory compared with the non-restructured approach. Therefore, taking into account the serious memory cost caused by a one-time restructuring, more extreme cases will cause a serious mismatch between the size of the feature map and the storage space. We will combine the OEC strategy to perform dataflow restructuring in batches to relieve memory pressure.
% However, such a memory sacrifice proves to be worthwhile, because the data locality benefit brought by the restructuring overweighes the additional memory cost and it can effectively accelerate the inference workflow (shown in \S\ref{sec-exp-at}). 


% OutC, InH, InW

% if(OutC >= Pn)
% {
% 	Partition by OutC;
% 	if (OutC % Pn == 0)
% 		return;
% 	else     //剩余 1～（Pn-1）个OutC
% 	{
% 		if(InH >= Pn)
% 		{
% 			Partition by InH;
% 			if (InH % Pn == 0)
% 				return;
% 			else     //剩余 1～（Pn-1）个InH
% 			{
% 				Partition by InW;
% 				if (InW % Pn == 0)
% 					return;
% 				else
% 					Randomly distribut by InW;
% 			}
% 		}else
% 			Randomly distribut by InH;
% 	}
% }else     //剩余 1～（Pn-1）个OutC
% {
% 	if(InH >= Pn)
% 	{
% 		Partition by InH;
% 		if (InH % Pn == 0)
% 			return;
% 		else     //剩余 1～（Pn-1）个InH
% 		{
% 			Partition by InW;
% 			if (InW % Pn == 0)
% 				return;
% 			else
% 				Randomly distribut by InW;
% 		}
% 	}else
% 		Randomly distribut by InH;
% }


% //上述伪代码合并后为下面的伪代码

% OutC, InH, InW

% if(OutC >= Pn)
% {
% 	Partition by OutC;
% 	if (OutC % Pn == 0)
% 		return;
% }
% //剩余 1～（Pn-1）个OutC
% if(InH >= Pn)
% {
% 	Partition by InH;
% 	if (InH % Pn == 0)
% 		return;
% 	else     //剩余 1～（Pn-1）个InH
% 	{
% 		Partition by InW;
% 		if (InW % Pn == 0)
% 			return;
% 		else
% 			Randomly distribut by InW;
% 	}
% }else
% 	Randomly distribut by InH;





\subsection{Distributed Inference} 
\label{sec-distributed-inference}
As the model size grows increasingly large, we envision that the inference workload can soon go beyond the capacity of single edge devices. Recent models, such as Bert (340M$\sim$481000M)~\cite{devlin2018bert} and GPT-3\cite{radford2018improving}(175000M), can hardly be used for single-device inference, making distributed inference become a necessity.



Driven by these current and future scenarios, we extend \sysname to leverage multiple devices for joint inference computation, and we call the distributed version of \sysname as \dsysname. The key idea of \dsysname is to incorporate both model-parallel computation and  parameter synchronization among multiple devices, to cut down the overall inference time. However, we note that, compared with \sysname, \dsysname may not achieve optimal inference time if it still follows the priorities of FMP to partition the feature map. Recall that FMP priorities \emph{outC}-based partition over \emph{inH}-/\emph{inW}-based partition (\S\ref{sec-ha-strategy}). This is because,  \emph{outC}-based partition can fully leverage the shared memory across different DSP units and avoid padding overheads due to  \emph{inH}-/\emph{inW}-based partition. However, when it comes to \dsysname, different edge devices do not shared memory, and it can hardly tell whether or not \emph{outC}-based partition can outperform \emph{inH}-/\emph{inW}-based partition. Therefore, \dsysname needs to balance two types of overheads, i.e., the communication overheads due to parameter synchronization and the computation overheads due to imbalanced partition. To make it, \dsysname starts a profiling period at the beginning and enumerates every possible combination of the three partition schemes towards each feature map involved in the inference, which can reach 6 different combinations at most, as shown in Figure~\ref{fig-branch-partition}.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{fig/branch-partition.pdf}
    \caption{Enumerating partition schemes in \dsysname}
    \label{fig-branch-partition}
    \vspace{-0.5cm}
\end{figure}

For every feature map, \dsysname picks the optimal partition scheme among the 6 branches. After the profiling, the optimal partition scheme have been determined for the entire inference process, and \dsysname uses it throughout all the inference work.

